Algorithmic Foundations of Deep Learning: Complexity-Theoretic Rates and a Characterization of Universal Approximation

Feedforward neural network (NN) expressivity is typically studied by emulating optimal basis-expansion schemes. While powerful, this perspective is incomplete: it primarily captures complexity through regularity, and therefore does not distinguish intuitively simple and complicated objects with comparable regularity, such as the square-root function and a typical Brownian path. The guiding message is that neural networks should be viewed not only as flexible basis functions, but also as models of computation. If a function is computable by a real-valued circuit over a prescribed elementary gate language, then it can be computed to comparable accuracy by an NN with explicit depth, width, and non-zero-parameter bounds controlled by the depth, width, gate count, and gate structure. Thus, neural-network complexity is not governed by regularity alone, but also by algorithmic complexity. We then show that any definable NN model satisfying a natural parallelization condition, allowing possibly multivariate non-linearities such as attention or layer normalization, is a universal approximator if and only if it contains a non-affine nonlinearity. The scope of our theory is illustrated by deducing universal approximation guarantees for continuous functions, minimax-optimal approximation guarantees for Besov classes, logarithmic-error complexity for holomorphic functions, and by showing that NNs can emulate numerical algorithms such as Newton-Raphson root finding and power iteration without architecture-specific arguments. Its precision is illustrated by shortest-path computation on $k$-vertex graphs: compiling the tropical dynamic-programming circuit yields NNs with O(log(1/{\epsilon})) non-zero parameters, exponentially improving in 1/{\epsilon} over the generic $O({\epsilon}^{-c k^2})$ Lipschitz-approximation scale, for a constant c>0.

==> Bookkeeping/0_AuthorsandInfo.tex <==
% \title{Decentralization Can Break The Curse of Dimensionality}
% \author{Anastasis Kratsios, Marc T. Law, Haitz Sáez de Oc\`{a}riz Borde, and Takashi Furuya}
% \date{October 2023}


% \title[Decentralization Breaks The Curse of Dimensionality]{Decentralization Breaks The Curse of Dimensionality}
% \usepackage{times}
% % Use \Name{Author Name} to specify the name.
% % If the surname contains spaces, enclose the surname
% % in braces, e.g. \Name{John {Smith Jones}} similarly
% % if the name has a "von" part, e.g \Name{Jane {de Winter}}.
% % If the first letter in the forenames is a diacritic
% % enclose the diacritic in braces, e.g. \Name{{\'E}louise Smith}

% % Two authors with the same address
% % \coltauthor{\Name{Author Name1} \Email{abc@sample.com}\and
% %  \Name{Author Name2} \Email{xyz@sample.com}\\
% %  \addr Address}

% % Three or more authors with the same address:
% % \coltauthor{\Name{Author Name1} \Email{an1@sample.com}\\
% %  \Name{Author Name2} \Email{an2@sample.com}\\
% %  \Name{Author Name3} \Email{an3@sample.com}\\
% %  \addr Address}

% % Authors with different addresses:
% \coltauthor{%
%  \Name{Anastasis Kratsios} \Email{kratsioa@mcmaster.ca}\\
%  \addr Address 1
%  \AND
%  \Name{Author Name2} \Email{xyz@sample.com}\\
%  \addr Address 2%
%  % \author{Anastasis Kratsios, Marc T. Law, Haitz Sáez de Oc\`{a}riz Borde, and Takashi Furuya}
% }

==> Bookkeeping/0_packages.tex <==
%%%%%%%%%%%%%%
%% Packages %%
%%%%%%%%%%%%%%
\usepackage{float}\usepackage{colortbl}
\usepackage{mathrsfs}
\usepackage{mathtools}
\usepackage{placeins}
\usepackage{xparse}
\usepackage{color}
\usepackage{comment}
\usepackage{natbib}

\usepackage{hyperref} 
    \hypersetup{
    	colorlinks = true,
    	linkcolor = blue,
    	anchorcolor = blue,
    	citecolor = blue,
    	filecolor = blue,
    	urlcolor = blue
    }

% Fonts and such
\usepackage{accents}
\def\baselinestretch{1}
% \renewcommand{\complement}{^c}
% \newcommand{\complement}{^c}
 \DeclareMathOperator{\deb}{deb}
 \DeclareMathOperator{\conv}{conv}

% Graphics and Figures
\usepackage{caption}
\usepackage{subcaption}
\usepackage{graphicx}

% TABLE Formatting
% \usepackage{tablefootnote}
\usepackage{adjustbox}
\usepackage{booktabs}
\raggedbottom
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\setlength\heavyrulewidth{0.3ex}
\renewcommand{\arraystretch}{1.25}
\usepackage{lscape}








%%% COLOURs and Commenting

%
%
%
%
%
%
\usepackage{marginnote}
\usepackage{xcolor}


